Predicting Decisions in Language Based Persuasion Games

Sender-receiver interactions, and specifically persuasion games, are widely researched in economic modeling and artificial intelligence. However, in the classic persuasion games setting, the messages sent from the expert to the decision-maker (DM) are abstract or well-structured signals rather than natural language messages. This paper addresses the use of natural language in persuasion games. For this purpose, we conduct an online repeated interaction experiment. At each trial of the interaction, an informed expert aims to sell an uninformed decision-maker a vacation in a hotel, by sending her a review that describes the hotel. While the expert is exposed to several scored reviews, the decision-maker observes only the single review sent by the expert, and her payoff in case she chooses to take the hotel is a random draw from the review score distribution available to the expert only. We also compare the behavioral patterns in this experiment to the equivalent patterns in similar experiments where the communication is based on the numerical values of the reviews rather than the reviews' text, and observe substantial differences which can be explained through an equilibrium analysis of the game. We consider a number of modeling approaches for our verbal communication setup, differing from each other in the model type (deep neural network vs. linear classifier), the type of features used by the model (textual, behavioral or both) and the source of the textual features (DNN-based vs. hand-crafted). Our results demonstrate that given a prefix of the interaction sequence, our models can predict the future decisions of the decision-maker, particularly when a sequential modeling approach and hand-crafted textual features are applied. Further analysis of the hand-crafted textual features allows us to make initial observations about the aspects of text that drive decision making in our setup

==> Language-Based-Persauision-Games- final version January 2022/inputs/defs.tex <==
\usepackage{xcolor}
\usepackage{gensymb} %for degree - in the acknowledge men
\usepackage{graphicx}
\usepackage{amsmath}
\usepackage{dsfont}
\usepackage{multirow} %merge rows in the table
\usepackage{amssymb} %triangleq


\newcommand{\alg}{\textsc{ALG}}
\newcommand{\mX}{\mathcal{X}}
\newcommand{\mC}{\mathcal{C}}
\newcommand{\mI}{\mathcal{I}}
\newcommand{\mF}{\mathcal{F}}
\newcommand{\mY}{\mathcal{Y}}
\newcommand{\mZ}{\mathcal{Z}}
\newcommand{\mH}{\mathcal{H}}
\newcommand{\mL}{\mathcal{L}}
\newcommand{\mA}{\mathcal{A}}
\newcommand{\mB}{\mathcal{B}}
\newcommand{\mO}{\mathcal{O}}
\newcommand{\mG}{\mathcal{G}}
\newcommand{\mD}{\mathcal{D}}
\newcommand{\mR}{\mathcal{R}}
\newcommand{\mM}{\mathcal{M}}
\newcommand{\mN}{\mathcal{N}}
\newcommand{\mS}{\mathcal{S}}
\newcommand{\mT}{\mathcal{T}}
\newcommand{\mW}{\mathcal{W}}
\newcommand{\ind}{\mathds{1}}
\newcommand{\zro}{\mathbb{0}}
%\newcommand{\E}{\mathbb{E}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\N}{\mathbb{N}}
\newcommand{\hr}{\mathcal{HR}}
\newcommand{\dpd}{\mathcal{DPD}}
\newcommand{\df}{\mathcal{DF}}
\newcommand{\ts}{\mathcal{TS}}
\newcommand{\hs}{\mathcal{HS}}
\newcommand{\defeq}{\stackrel{\text{def}}{=}}
\newcommand{\vc}{\textnormal{VCdim}}
\newcommand{\pdim}{\textnormal{Pdim}}
\newcommand{\poly}{\text{poly}}
\newcommand{\Var}{\mathrm{Var}}


\newcommand{\tmS}{\tilde{\mathcal{S}}}
\newcommand{\tmX}{\tilde{\mathcal{X}}}
\newcommand{\tmY}{\tilde{\mathcal{Y}}}
\newcommand{\tmZ}{\tilde{\mathcal{Z}}}
\newcommand{\tmD}{\tilde{\mathcal{D}}}
\newcommand{\tmI}{\tilde{\mathcal{I}}}
\newcommand{\tmF}{\tilde{\mathcal{F}}}
\newcommand{\tz}{\tilde{z}}
\newcommand{\tw}{\tilde{w}}
\newcommand{\tpi}{\tilde{\pi}}


\newcommand{\inprod}[2]{\langle\, #1,#2\rangle}
\citepunct{}{\&}{and}{, }{; }{, }{}{}{.}
\newcommand{\citep}[1]{(\cite{#1})}
\newcommand{\citet}[1]{\citeauthor{#1}~(\citeyear{#1})}


%\theoremstyle{plain}
\newtheorem{claim}{Claim}
\newtheorem{observation}{Observation}
\newtheorem{question}{Question}
\numberwithin{claim}{section} 
\numberwithin{observation}{section} 
\numberwithin{question}{section} 



\newcommand\bl[1]{\boldsymbol{ #1 } }
\newcommand{\norm}[1]{\left\lVert#1\right\rVert}
%\DeclarePairedDelimiter\abs{\lvert}{\rvert}%
\newcommand\abs[1]{\left| #1  \right|}
\DeclareMathOperator*{\argmin}{arg\,min} %argmin
\DeclareMathOperator*{\argmax}{arg\,max} %argmax
\DeclareMathOperator{\sgn}{sgn}
\DeclareMathOperator{\E}{\mathbb{E}}
\DeclareMathOperator{\pr}{\mathbb{P}}
\DeclareMathOperator{\sign}{sign}
\DeclareSymbolFont{rsfs}{U}{rsfs}{m}{n}
\DeclareSymbolFontAlphabet{\mathscrsfs}{rsfs}
\DeclareUnicodeCharacter{2212}{-}
